Feasibility of Transfer Learning: A Mathematical Framework

Transfer learning is a popular paradigm for utilizing existing knowledge from previous learning tasks to improve the performance of new ones. It has enjoyed numerous empirical successes and inspired a growing number of theoretical studies. This paper addresses the feasibility issue of transfer learning. It begins by establishing the necessary mathematical concepts and constructing a mathematical framework for transfer learning. It then identifies and formulates the three-step transfer learning procedure as an optimization problem, allowing for the resolution of the feasibility issue. Importantly, it demonstrates that under certain technical conditions, such as appropriate choice of loss functions and data sets, an optimal procedure for transfer learning exists. This study of the feasibility issue brings additional insights into various transfer learning problems. It sheds light on the impact of feature augmentation on model performance, explores potential extensions of domain adaptation, and examines the feasibility of efficient feature extractor transfer in image classification.

==> literature.tex <==
\section{Literature Review}

Transfer learning is based on a straightforward concept: utilizing knowledge gained from a well-researched learning problem, called the source task, to enhance the performance of a new, similar learning problem, referred to as the target task.  This approach has proven successful in various fields, such as natural language processing \cite{ruder2019transfer, devlin-etal-2019-bert, sung2022vl}, sentiment analysis \cite{jiang2007instance, deng2013sparse, liu2019survey}, computer vision \cite{deng2009imagenet, long2015learning, ganin2016domain, wang2018deep}, activity recognition \cite{cook2013transfer, wang2018stratified}, medical data analysis \cite{zeng2019automatic, wang2022transfer, kim2022transfer}, bioinformatics \cite{hwang2010heterogeneous}, finance \cite{leal2020learning,rosenbaum2021deep}, recommendation systems \cite{pan2010transfer, yuan2019darec}, and fraud detection \cite{lebichot2020deep}. Numerous review papers also provide further insight \cite{survey1,tan2018survey,zhuang2020comprehensive}.

Nonetheless, the performance improvement from transfer learning can be inconsistent, with the potential for negative transfer in some cases \cite{wang2019characterizing}. Factors that influence these outcomes include the similarity between the source and target tasks, the design of the model architectures, and the specific transfer learning method employed. To understand transfer learning performance from a theoretical perspective, there is increasing interest in proposing mathematical frameworks and developing transferability measures or generalization bounds that bridge the gap between the theory and practice of transfer learning.




==> office31.tex <==
\section{Numerical Experiments with Office-31}\label{sec:image_experiment}
In this section, we will demonstrate the correlation between the performance of the transfer learning scheme \eqref{eq: doub-trans} and the transfer risk \eqref{defn: trans-bene}, through numerical experimentation using the Office-31 dataset for image classification.  

\subsection{Experiment Set-up}
Recall the neural network architecture for the experiment introduced in Section \ref{subsec:example}. For each pair of the source and the target tasks, the source model is first trained using the source data, and then the fully connected layer of the pretrained model is fine tuned using half of the target data. The performance of the model is measured by the classification accuracy using the remaining of the target data.

\paragraph{Transfer risk.} Now let us define the explicit form of transfer risk for this example. Fix a source-target pair $(S,T)$. Recall that the input transport risk $\Ef^I$ is a constant since the input transport set $\mathbb{T}^X$ is a singleton set. More specifically, we define the input transport risk as 
\begin{equation}\label{eqn:office_input}
    \Ef^I:=\mathcal{W}_1(Law(X_S), Law(X_T)),
\end{equation}
which is the Wasserstein-1 distance between the empirical distribution of (resized) source images $Law(X_S)$ and the empirical distribution of (resized) target images $Law(X_T)$. Meanwhile, for any $f_{ST}\in\mathcal{I}$ \eqref{eqn:nnclass}, we define the output transport risk as $\Ef^O(f_{ST})=\mathcal{W}_1({\mathbb{P}}_{ST}, {\mathbb{P}}_T).$
Furthermore, as discussed in Section \ref{subsec:example_revisited}, the transfer risk is given by 
\begin{equation}\label{eqn:office_risk}
    \mathcal{C}(S,T)=C(\Ef^I,\min_{f_{ST}\in\mathcal{I}}\Ef^O(f_{ST})),
\end{equation}
for some function $C:\R^2\to\R$ satisfying the regularity conditions in Definition \ref{defn: trans-bene}. Note the the optimal target distribution $\mathbb{P}_T$ in the definition of $\Ef^O(f_{ST})$ is unknown {\it a priori}. Thus, as suggested by Proposition \ref{lem: w-heur}, we approximate $\Ef^O(f_{ST})$ by $\mathcal{W}_1({\mathbb{P}}_{ST}, Law(Y_T))$. Denote the approximated output transfer risk as 
\begin{equation}\label{eqn:office_out_risk}
    \widehat{\Ef}^O=\min_{f_{ST}\in\mathcal{I}}\mathcal{W}_1({\mathbb{P}}_{ST}, Law(Y_T)).
\end{equation}
Finding $\widehat{\Ef}^O$ \eqref{eqn:office_out_risk} is an optimization problem over a neural network function class $f_{ST}\in\mathcal{I}$ \eqref{eqn:nnclass}, which is solved by gradient descent in the numerical experiment. Finally, the (approximated) transfer risk is obtained by plugging $\widehat{\Ef}^O$ into \eqref{eqn:office_risk}. 


\subsection{Numerical Result}
Three different domains in Office-31 (A, D, and W) lead to $3\times 2=6$ source-target pairs in total. The accuracy, the input transport risk $\Ef^I$ \eqref{eqn:office_input}, and the output transport risk $\widehat\Ef^O$ \eqref{eqn:office_out_risk} for each pair of source and target tasks are reported in the first three rows of Table \ref{tab:office31}. Here the input transport risk is rescaled by a constant factor to achieve the same scale as the other metrics.

In order to compute the transfer risk $\mathcal{C}$ in \eqref{eqn:office_risk} given $\Ef^I$ in \eqref{eqn:office_input} and $\widehat\Ef^O$ in \eqref{eqn:office_out_risk}, an appropriate form of function $C$ in \eqref{eqn:office_risk} need to be determined. In this experiment, we search $C$ from the class of second order polynomials, so as to maximize the (absolute value of) correlation between the transfer learning accuracy and the transfer risk. In particular, we define the risk in the following form:
\begin{equation}\label{eqn:office_risk_exact}
    \mathcal{C}(S,T)=0.31\cdot\Ef^I+0.92\cdot\left(\widehat\Ef^O\right)^2.
\end{equation}
Transfer risks for all source-target pair are reported in the last row of Table \ref{tab:office31}.

\begin{table}[H]
  \centering
    \begin{tabular}{c|cccccc}
    \toprule
    \toprule
    \textbf{Metric\textbackslash{}Task} & \textbf{A-W}   & \textbf{A-D}   & \textbf{W-A}   & \textbf{W-D}   & \textbf{D-A}   & \textbf{D-W} \\
    \midrule
    \textbf{Accuracy} & 80.9\% & 83.1\% & 66.9\% & 94.5\% & 66.6\% & 87.8\% \\
    \midrule
    \textbf{Input Risk} & 0.181 & 0.263 & 0.181 & 0.148 & 0.263 & 0.148 \\
    \midrule
    \textbf{Output Risk} & 0.428 & 0.380 & 0.545 & 0.084 & 0.543 & 0.412 \\
    \midrule
    \textbf{Transfer Risk} & 0.224 & 0.214 & 0.330 & 0.052 & 0.353 & 0.201 \\
    \bottomrule
    \bottomrule
    \end{tabular}
  \caption{Accuracy and transfer risk.}
  \label{tab:office31}
\end{table}

\paragraph{Accuracy v.s. transfer risk.} Figure \ref{fig:office31} demonstrates a significant negative correlation between the transfer learning accuracy and the transfer risk: the higher the risk, the lower the transfer learning accuracy. For example, it can be observed from Figure \ref{fig:office31} that transfer learning between DSLR and Webcam (D-W or W-D) results in low risk and high accuracy; while transfer learning from those domains to Amazon (D-A or W-A) is risky and suffers from low accuracy. Those numerical findings demonstrate the potential of transfer risk as an informative metric for the effectiveness of transfer learning task.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.6\textwidth]{figures/acc_risk.png}
    \caption{Accuracy and transfer risk.}
    \label{fig:office31}
\end{figure}

\paragraph{Computational benefit of  transfer risk.}  

In this numerical experiment on the Office-31 dataset, assessing transfer risk is computationally efficient and guaranteed by the early-stopping trick in deep learning: for each source-target pair, the optimization problem \eqref{eqn:office_out_risk} is solved by running the gradient descent for a small and fixed number ($\sim$10) of epochs, while the transfer learning problem is solved until the accuracy converges, which may take up to  100 epochs. This early stopping trick is essentially equivalent to shrinking the search space of the output mapping from  $\mathbb{T}^Y$ in \eqref{eqn:nnclass} to some smaller class of neural networks $\mathbb{T}_0^Y\subset\mathbb{T}^Y$. 

Indeed, as emphasized in Section \ref{subsec:def_risk}, computing transfer risk \eqref{eqn:risk} is to solve an optimization problem  over the sets $\mathbb{T}^X_0$ and $\mathbb{T}^Y_0$, which can be much smaller than the function classes $\mathbb{T}^X$ and $\mathbb{T}^Y$ involved in the transfer learning problem \eqref{eq: doub-trans}. This reduction of the function classes demonstrates the potential and benefit of adopting transfer risk for  computational efficiency:  one can first perform the much easier computing task of the transfer risk, and then assess whether or not to resort to the full-scale and more computationally intense form of transfer learning.




==> transfer_risk.tex <==
\section{Transfer risk for transfer learning}
The procedure of finding the solution $(T^{X,*},T^{Y,*})$ to the optimization problem \eqref{eq: doub-trans} is often referred to as fine-tuning in the literature of transfer learning. It is to choose some initial transport mappings $T^X_0\in\T^X_0\subset\T^X$ and $T^Y_0\in\T^Y_0\subset\T^Y$ to derive an intermediate model $f_{ST}\in A_T$ with
\begin{equation}\label{eq: int-model}
    f_{ST}(x)=T^Y_0(x, (f_S^*\circ T^X_0)(x)),\quad \forall x\in\XCal_T,
\end{equation}
with the set of possible intermediate models denoted as
\begin{equation}\label{eq: int-set}
    \ICal=\left\{T^Y_0(\cdot, (f_S^*\circ T^X_0)(\cdot))\big|T^X_0\in\T^X_0, T^Y_0\in\T^Y_0\right\}.
\end{equation}

Given the mathematical framework and after the feasibility analysis of transfer learning, we now propose  a novel notion of {\it transfer risk}, to analyze the effectiveness and the appropriateness of transfer learning over the set of all intermediate models $\ICal$ given by \eqref{eq: int-set}.
 
\subsection{Transfer risk}\label{subsec:def_risk}
The idea is to re-interpret the transfer learning framework \eqref{eq: tl-fw} in a sequential manner:  the mapping $T^X$ first transports $Law(X_T)$ to some probability distribution $Law(T^X(X_T))$; then, applying the pretrained model $f^*_S$ for the optimization problem \eqref{eq: obj-s} yields the distribution $\tilde\pbm_S=Law(f^*_S(T^X(X_T)))$.
%\in\mathcal{P}(\YCal_S)$. 
Finally, an output transport mapping $T^Y$, together with  the target input $X_T$,  transports the distribution $\tilde\pbm_S$ to $\pbm_T$. 
That is,  the transfer learning scheme can be viewed as the composition of the following two steps.
\begin{enumerate}
    \item (Psuedo) Domain adaption, which can also be seen as optimal transport from $Law(X_T)$ to $Law(X_S)$.
    \item Optimal transport from $\tilde\pbm_S=Law(f^*_S(T^X(X_T)))$ to $\pbm_T$ over $T^Y$. 
    %with transport cost given by the regret function $L_T(T^Y(\cdot,f_S(T^X(\cdot)));X_T,Y_T)-L_T(f_T;X_T,Y_T)$.
\end{enumerate}

In other words, in parallel to the three-step procedure in transfer learning, there are two major sources of transfer risk for a fixed intermediate model $f_{ST}\in\ICal$:  the risk that measures the mismatch  between the output distributions of the intermediate model $f_{ST}$ and the optimal target model $f_T^*$, and the risk reflecting the difference between the transported target input and the source input. 

Let us first define the risk associated  the output transport mapping.
\begin{defn}[Output transport risk]\label{defn:outputrisk}
Let \(\Ef^O:A_T\to\R\) be a real-valued function on the set of target models. For any \(f_{ST}\in\ICal\subset A_T\), $\Ef^O(f_{ST})$ is called an output transport risk of intermediate model $f_{ST}$ if it  satisfies
    \begin{enumerate}
        \item $\Ef^O(f_{ST})\geq 0$, i.e., transfer learning always incurs a non-negative effort;
        \item $\Ef^O(f_{ST})=0$ if and only if $\pbm_T=\pbm_{ST}$, where $\pbm_T:=Law(f_{T}(X_T))$ and $\pbm_{ST}:=Law(f_{ST}(X_T))$. That is, the output transport risk vanishes when the intermediate model $f_{ST}$ completely recovers the distribution of the optimal target task.
    \end{enumerate}
\end{defn}

Clearly, the smaller this output risk, the more effective the transfer scheme with the intermediate model $f_{ST}$. 

We next define the risk associated with the input transfer.
\begin{defn}[Input transfer risk]\label{defn: inputrisk}
Let \(\Ef^I:\T^X\to\R\) be a real-valued function on the set of input transport mappings. Given an import transport mapping $T^X_0\in\T^X_0\subset \T^X$, $\Ef^I(T^X_0)$ is called an input transport risk if it  satisfies
    \begin{enumerate}
        \item $\Ef^I(T^X_0)\geq 0$, i.e., transfer learning always incurs a non-negative effort;
        \item $\Ef^I(T^X_0)=0$ if and only if $T^X_0\#Law(X_T)=Law(X_S)$. 
    \end{enumerate}
\end{defn}
The smaller this input risk, the higher the similarity between the transported target input $T^X_0(X_T)$ and the source input $X_S$. 



%this is a case where relaying to the source optimization problem is the most beneficial. 

% To solve this optimization problem, one can choose some initial transport mappings $T^X_0\in\T^X_0\subset\T^X$ and $T^Y_0\in\T^Y_0\subset\T^Y$ to derive an intermediate model $f_{ST}\in A_T$ with
% \begin{equation}\label{eq: int-model}
%     f_{ST}(x)=T^Y_0(x, (f_S^*\circ T^X_0)(x)),\quad \forall x\in\XCal_T,
% \end{equation}
% with the set of possible intermediate models denoted as
% \begin{equation}\label{eq: int-set}
%     \ICal=\left\{T^Y_0(\cdot, (f_S^*\circ T^X_0)(\cdot))\big|T^X_0\in\T^X_0, T^Y_0\in\T^Y_0\right\}.
% \end{equation}


Note  that these definitions of risks involve the sets of initial transport mappings $\T^X_0$ and $\T_0^Y$, instead of the sets of all possible transport mappings $\T^X$ and $\T^Y$. These reduced sets allow for efficient evaluation of transfer risk prior to starting the full-scale transfer learning.

Both the input transfer risk and the output transfer risk are functions characterizing the divergence between probability distributions, and their exact forms can be task dependent.  Nevertheless,  there is a key difference between these two forms of risks:  in the output transport risk, $\pbm_T$, the output distribution of the optimal target model, is {\it unknown}, and no prior knowledge about $f_T^*$ is assumed. 
Therefore, analyzing the output transport risk is decisively more complicated.
See more detailed discussions in Section \ref{sec:divergence}.

We are now ready to propose the notion of  {\it transfer risk}  by considering all intermediate models in $\ICal$, in order to  measure the effectiveness of a transfer learning framework \eqref{eq: doub-trans}.
\begin{defn}[Transfer risk]\label{defn: trans-bene}
For a transfer learning procedure characterized by the 6-tuple ${(S,T,\T^X,\T^X_0,\T^Y,\T^Y_0)}$  in \eqref{eq: doub-trans}, the transfer risk of the transfer learning framework \eqref{eq: doub-trans} from source task $S$ to target task $T$ is defined as
\begin{equation}\label{eqn:risk}
\CCal(S,T)=\inf_{f_{ST}\in\ICal}\CCal(S,T|f_{ST}).
\end{equation}
Here, for a given $f_{ST}=T^Y_0(\cdot, (f_S^*\circ T^X_0)(\cdot))\in\ICal$, $\CCal(S,T|f_{ST})$ is called  model-specific transfer risk such that $\CCal(S,T|f_{ST})\ge 0$ with the following properties:
\begin{enumerate}
    \item Let $C:\R\times\R\to\R$ with $C(0,0)=0$. $\CCal(S,T|f_{ST})=C(\Ef^O(f_{ST}),\Ef^I(T^X_0))$ is non-decreasing in $\Ef^O(f_{ST})$ under any fixed $\Ef^I(T^X_0)$ and non-decreasing in $\Ef^I(T^X_0)$ under any fixed $\Ef(f_{ST})$; 
    \item $\CCal(S,T|f_{ST})$ is Lipschitz  in the sense that for any other transfer problem characterized by $(\bar S,\bar T,\bar\T^X,\bar\T_0^X,\bar\T^Y,\bar\T_0^Y)$ and one of its intermediate models $\bar f_{ST}=\bar T^Y_0(\cdot, (\bar f_S^*\circ \bar T^X_0)(\cdot))\in\bar\ICal$, there exists a constant $L>0$ such that 
    \[\begin{aligned}|\CCal(S,T|f_{ST})-\CCal(\bar S,\bar T|\bar f_{ST})|&\leq L(|\Ef^O(f_{ST})-\Ef^O(\bar f_{ST})|\\
    &\qquad\qquad+|\Ef^I(T^X_0)-\Ef^I(\bar T^X_0)|).\end{aligned}\]
\end{enumerate}
\end{defn}
The expression of this Lipschitz property in Definition \ref{defn: trans-bene} is to emphasize the dependence of transfer risk on a given transfer learning problem. This Lipschitz property is satisfied when the function $C$ in Definition \ref{defn: trans-bene} is Lipschitz continuous. 

One simple example of the model-specific transfer risk is
\begin{equation}\label{eq: risk-ln}
    \CCal^\lambda(S,T|f_{ST})=\Ef^O(f_{ST})+\lambda \Ef^I(T^X_0),
\end{equation}
where $\lambda>0$ is a pre-specified parameter modulating the weight of the input transport in the transfer learning problem \eqref{eq: tl-fw}. 

Transfer risk in Definition \ref{defn: trans-bene} unifies the analysis of the risk from both the input and the output transport mappings. It allows for studying  the trade-off between them. Moreover, two of its key components, the input and the output transfer risks in Definitions \ref{defn: inputrisk} and \ref{defn:outputrisk} generalize earlier works on transferability. For instance, the $\mathcal{H}$-score proposed in \cite{bao2019information} addresses transferability of a particular classification setting and can be incorporated into the output transfer risk in Definition \ref{defn:outputrisk}. Earlier works on the relation between source and target inputs such as \cite{saenko2010adapting, ganin2016domain, long2014transfer} correspond to the special case in Definition \ref{defn: inputrisk} with $T^X_0$ being the identity mapping. 

Furthermore, one can establish the following properties of transfer risk: a)  there is zero transfer risk if the source and the target tasks are identical; and b) transfer risk is continuous in the input distribution and robust with respect to the  pretrained model. The continuity of the transfer risk in terms of the changes in the input and the pretrained model is useful to exclude {\it a priori} inappropriate source tasks when compared against existing viable source tasks. 

\subsection{Properties of transfer risk}\label{subsec: property}

In this section, the mathematical properties of transfer risk \eqref{eqn:risk} will be studied under mild assumptions. In the following discussion, we will fix a target task $T$ and explore how transfer risk is affected by the choice of source task $S$.

There are two vital pieces of information obtained from the source task $S$ based on the optimization problem in \eqref{eq: doub-trans}, and  transfer risks in \eqref{eqn:risk}. One is the probability distribution of source input $Law(X_S)$, and the other is the pretrained model $f_S^*$ in \eqref{eq: obj-s}  Therefore, we can characterize source task $S$ by $(Law(X_S),f_S^*)$. More specifically, given a  target task $T$ and the source input and output spaces $\XCal_S$ and $\YCal_S$, we can define a corresponding set of pretrained source tasks $\SCal\subset\mathcal{P}(\XCal_S)\times A_S$. Without ambiguity on the target task $T$, we denote $\CCal(S,T)=\CCal(S)=\CCal(\mu,f)$ for any $S=(\mu,f)\in\SCal$. For the set of probability measures over $\XCal_S$, $\mathcal{P}(\XCal_S)$, we can adopt a metric function $D:\mathcal{P}(\XCal_S)\times \mathcal{P}(\XCal_S)\to\R$. Then for the set of functions $A_S$, fix a sufficiently large constant $M>0$ and define the following metric: $\forall f_1,f_2\in A_S,$
\[d_M(f_1,f_2):=\min\{M,\sup_{x\in\XCal_S}\|f_1(x)-f_2(x)\|_{\YCal_S}\}.\]
Then for any $S_1,S_2\in\SCal$ such that $S_1=(\mu_1,f_1)$ and $S_2=(\mu_2,f_2)$, define
\begin{equation}\label{eqn:d_s}
    d_S(S_1,S_2):=D(\mu_1,\mu_2)+d_M(f_1,f_2).
\end{equation}


It is easy to verify that $d_S$ is a metric over $\SCal$. 

In the following discussion on continuity, the next assumption is necessary. Assumption \ref{ass:D} ensures that the choice of input transfer risk is consistent with the metric $d_S$ in \eqref{eqn:d_s} defined between source tasks.

\begin{asp}\label{ass:D}
    For any input transport mapping $T^X_0\in\mathbb{T}^X_0$, assume the input transfer risk $\Ef^I(T^X_0)$ take the form  $\Ef^I(T^X_0):=D(T^X_0\#Law(X_T),Law(X_S))$, where $D:\mathcal{P}(\XCal_S)\times \mathcal{P}(\XCal_S)\to\R$ is the distance function appearing in \eqref{eqn:d_s}.
\end{asp}

By definition, the following degenerate case holds immediately.
\begin{prop}[Zero transfer risk]
    Suppose $\XCal_T=\XCal_S$, $\YCal_T=\YCal_S$ and the target task $T\in\SCal$. Then $\CCal(T)=0$.
\end{prop}


Now, we consider source tasks $S_1,S_2\in\SCal$ that differ only in the input distribution, i.e., $S_f^1=(\mu_1,f)$ and $S_f^2=(\mu_2,f)$. Then we have the following continuity property for $\CCal$.
\begin{prop}[Continuity in input distribution]\label{lem: cont-distr}
    Assume Assumption \ref{ass:D}. Fix $f\in A_S$. $\CCal(\cdot, f)$ is continuous on $(\mathcal{P}(\XCal_S),D)$.
\end{prop}

\begin{proof}[Proof of Proposition \ref{lem: cont-distr}]
Fix an arbitrary $\epsilon>0$. Take any $\mu\in\mathcal{P}(\XCal_S)$.
Then we first establish the lower semi-continuity: For any $T^X_0\in\T_0^X$ and $T_0^Y\in\T_0^Y$, let $f_{I}$ denote the corresponding intermediate model from source model $f$. By Definition \ref{defn: trans-bene}, we have
\[\CCal(\mu,f)-\frac{1}{2}\epsilon<\CCal(\mu,f|f_{I}).\]
By triangle inequality of $D$ and the Lipschitz property of $\CCal(\mu,f|f_I)$, take $\delta=\frac{\epsilon}{2L}$ for any $\mu'\in B_\delta(\mu)\subset \mathcal{P}(\XCal_S)$,
\[\CCal(\mu,f|f_{I})\leq \CCal(\mu',f|f_{I})+L\delta.\]
Notice that the choice of $\delta$ is independent of $T_0^X$ and $T_0^Y$. Therefore, 
\[\CCal(\mu,f)-\epsilon<\CCal(\mu',f;f_{I})\Rightarrow \CCal(\mu,f)-\epsilon<\CCal(\mu',f).\]

Now we show the upper semi-continuity.  From the infimum nature of $\CCal$, there exists $\bar T_0^X\in\T_0^X$ and $\bar T_0^Y\in\T_0^Y$, with corresponding intermediate model $\bar f_I$, such that 
\[\CCal(\mu,f|\bar f_{I})<\CCal(\mu,f)+\frac{1}{2}\epsilon.\]
Again, by triangle inequality of $D$ and the Lipschitz property of $\CCal(\mu,f|f_I)$, take $\delta=\frac{\epsilon}{2L}$ for any $\mu'\in B_\delta(\mu)\subset \mathcal{P}(\XCal_S)$,
\[\CCal(\mu,f|\bar f_{I})\geq \CCal(\mu',f|\bar f_{I})-\delta.\]
Then we have 
\[\CCal(\mu',f)\leq \CCal(\mu',f|\bar f_{I})<\CCal(\mu,f)+\epsilon.\]
Hence, we conclude that $\CCal(\cdot, f)$ is continuous on $(\mathcal{P}(\XCal_S),D)$.
\end{proof}

This proposition shows that transfer risk will change continuously along with any modification in source input. Its proof indicates that the sensitivity of transfer risk with respect to the change in source input distribution depends on the Lipschitz constant $L$ of $\CCal$. Therefore, one can modulate this sensitivity by carefully designing the $C$ function in Definition \ref{defn: trans-bene}. For instance, for linear transfer risk $\CCal^\lambda$ in \eqref{eq: risk-ln}, the sensitivity can be controlled by varying the value of $\lambda$.

Next, consider source tasks $S_1,S_2\in\SCal$ that differ only in the pretrained model, i.e., $S_\mu^1=(\mu,f_1)$ and $S_\mu^2=(\mu,f_2)$. Then we have  the robustness of the transferability in terms of  the continuity of $\CCal(\mu,\cdot)$ in pretrained model $f\in(A_S,d_M)$. 

\begin{prop}[Continuity in pretrained model]\label{lem: cont-f} 
Assume Assumption \ref{ass:D}, and assume that there exists a constant $L>0$ such that for any $T_0^Y\in\T_0^Y$, 
\[T_0^Y(x_1,y_1)-T_0^Y(x_2,y_2)\leq L\left(\|x_1-x_2\|_{\XCal_T}+\|y_1-y_2\|_{\YCal_S}\right),\]
for all $(x_1,y_1),(x_2,y_2)\in\XCal_T\times\YCal_S$.
Assume also that there exist  some $L'>0$ and $p\geq1$ such that the output transfer risk satisfies
    \[\left|\Ef^O(h_1)-\Ef^O(h_2)\right|\leq L'\mathcal{W}_p(h_1\#Law(X_T),h_2\#Law(X_T))^p\]
    for all $h_1,h_2\in\mathcal I$. 
    Then $\CCal(\mu,\cdot)$ is continuous on $(A_S,d_M)$ for any fixed $\mu\in\mathcal{P}(\XCal_S)$.
\end{prop}

\begin{proof}[Proof of Proposition \ref{lem: cont-f}]
Take any $T_0^X\in\T_0^X$ and $T_0^Y\in\T_0^Y$. For any $f_1,f_2\in(A_S,d_M)$, denote their corresponding intermediate model as $f_I^1$ and $f_I^2$, respectively. Then we have
\[\begin{aligned}
&|\Ef^O(f_I^1)-\Ef^O(f_I^2)|\\
&\quad\leq L'\mathcal{W}_p(f_I^1\#Law(X_T),f_I^2\#Law(X_T))^p\\
&\quad=L'\inf_{\pi\in\Pi(f_I^1\#Law(X_T),f_I^2\#Law(X_T))}\int_{\YCal_T\times\YCal_T}\|x-y\|_{\YCal_T}^p\pi(dx,dy)\\
&\quad\leq L'\inf_{\gamma\in\Pi(Law(X_T),Law(X_T))}\int_{\XCal_T\times\XCal_T}\|T_0^Y(x,f_1(T_0^X(x)))-T_0^Y(y,f_2(T_0^X(y)))\|_{\YCal_T}^2\pi(dx,dy)\\
&\quad\leq 2^{p-1}L^pL'\left[\inf_{\gamma\in\Pi(Law(X_T),Law(X_T))}\int_{\XCal_T\times\XCal_T}\|x-y\|_{\XCal_T}^pd\pi(dx,dy)+d_M(f_1,f_2)^p\right]\\
&\quad=2^{p-1}L^pL'\left[\mathcal{W}_p(Law(X_T),Law(X_T))^p+d_M(f_1,f_2)^p\right]=2^{p-1}L^pd_M(f_1,f_2)^p.
\end{aligned}\]
The rest of the proof is similar to that of Proposition \ref{lem: cont-distr}.
\end{proof}

This proposition shows that transfer risk will change continuously along with the modification in the pretrained model. As seen from the proof, the sensitivity of transfer risk with respect to the change in pretrained model is determined by three factors: (1) the Lipschitz constant inherited from the $C$ function in Definition \ref{defn: trans-bene}, (2) the choice of output transport risk $\Ef^O$, and (3) the family of output transport mappings $\T_0^Y$. In practice, one may control the sensitivity of the transfer risk through careful choices of those quantities.

%In practice, the structure of $\T_0^Y$ is determined by the setup of the transfer learning problem, while the design of $C$ function and the selection of appropriate output risk $\Ef^O$ can be adjusted in the evaluation of transferability. 

Propositions \ref{lem: cont-distr} and \ref{lem: cont-f} lead to the following results.
\begin{prop}
    \label{thm: cont}
    Suppose the conditions in Proposition \ref{lem: cont-f} hold. Then the transfer risk $\CCal$ as in Definition \ref{defn: trans-bene} is continuous on $(\SCal, d_S)$.
\end{prop}

Propositions \ref{lem: cont-distr} -- \ref{thm: cont} reveals that under a given target task, transfer risk is continuously influenced by both the changes in the source input and the pretrained model. Therefore, transfer risk is to evaluate the suitability of performing transfer learning and the  appropriate choice of given source tasks for a  target task.


\subsection{Examples}\label{subsec:example_revisited}
We now revisit some examples in Section \ref{subsec:example} and their associated transfer risks based on Definition \ref{defn: trans-bene}. In particular, we will illustrate how the two key components of the transfer risk, namely, the input transport risk $\Ef^I$ and the output transport risk $\Ef^O$, are embedded in transfer learning for a given intermediate model $f_{ST}$.

\paragraph{Transfer risk in domain adaption.}\label{subsec: DA}
Recall the domain adaptation problem in Section \ref{subsec:example}, and consider the case where the transfer risk is independent of the output transport risk, i.e., the input risk $\Ef^I(T^X_0)$ completely determine the transfer risk:
\[\CCal(S,T|f_{ST})=\Ef^I(T^X_0).\] 
In this case, there exists a one-to-one input mapping $T^X\in\T^X_0$ such that $T^X(X_T)=X_S$ almost surely, implying $T^X\#Law(X_T)=Law(X_S)$ and consequently $\CCal(S,T)=\CCal(S,T|f^*_S\circ T^X)=\Ef^I(T^X)=0$. Therefore, vanishing input transport risk is a necessary condition for the domain adaptation framework to hold. Thus, the input transport risk may be adopted to check the viability of domain adaptation on certain tasks.

\paragraph{Transfer risk in image classification.}
Recall the image classification problem introduced in Section \ref{subsec:example}. Fix a source task $S$ and a target task $T$. Since the input transport set $\mathbb{T}^X$ in this problem is a singleton set, the input transport risk $\Ef^I$ is a constant depending on $Law(X_S)$ and $Law(X_T)$, with the output transport risk  denoted as $\Ef^O(f_{ST})$ for any $f_{ST}\in\mathcal{I}$ in \eqref{eqn:nnclass}. By Definition \ref{defn: trans-bene}, the model-specific transfer risk $\mathcal{C}(S,T|f_{ST})=C(\Ef^I, \Ef^O(f_{ST}))$ for some appropriate function $C:\R^2\to\R$ satisfying conditions stated in Definition \ref{defn: trans-bene}. In particular, since the function $C$ is non-decreasing with respect to $\Ef^O(f_{ST})$, minimizing $\mathcal{C}(S,T|f_{ST})$ over $f_{ST}\in\mathcal{I}$ is equivalent to minimizing $\Ef^O(f_{ST})$ over $f_{ST}\in\mathcal{I}$:
\begin{equation*}
    \argmin_{f_{ST}\in\mathcal{I}}\mathcal{C}(S,T|f_{ST})=\argmin_{f_{ST}\in\mathcal{I}}\Ef^O(f_{ST}).
\end{equation*}
And consequently,
\begin{equation*}
    \mathcal{C}(S,T)=\min_{f_{ST}\in\mathcal{I}}\mathcal{C}(S,T|f_{ST})=C(\Ef^I,\min_{f_{ST}\in\mathcal{I}}\Ef^O(f_{ST})).
\end{equation*}


\subsection{Transfer risk and choices of divergence functions}
\label{sec:divergence}
Clearly, different learning tasks may require  different choices of divergence functions for assessment of transfer risk. In this section, we present two forms of transfer risks
based on two divergence functions, and analyze their properties and relations.

\paragraph{KL-based output transport risk.} For learning tasks such as the classification problem, one may use  cross-entropy as the loss function. 

Specifically, let $\pbm_T=\tilde\pbm_T+\pbm_0$ be its unique Lebesgue decomposition, i.e., for any measurable set $B\subset\YCal_T$, there exists some  function $h_{ST}:\YCal_T\to\R^+$ such that
$\tilde\pbm_T(B)=\int_Bh_{ST}d\pbm_{ST}$, with $\pbm_0$ singular with respect to $\pbm_{ST}$. Then the KL-based output risk can be  defined as
    \[
    \Ef^O_\text{KL}(f_{ST}):=D_\text{KL}(\tilde\pbm_T\|\pbm_{ST})+{H}(\pbm_0),
    \]
where $H(\pbm_0)$ is the entropy function of $\pbm_0$. 

 


\begin{prop}\label{lem: kl-heur}
    For a classification problem over $K\in\mathbb{N}$ classes with cross entropy as the training loss,  for any $f_{ST}\in\mathcal{I}$, 
    \begin{eqnarray*}
    \sum_{i=1}^K\log p_{ST}(i) \leq H(\pbm_T,\pbm_{ST})-H(Law(Y_T),\pbm_{ST}) \leq -\sum_{i=1}^K\log p_{ST}(i),
    \end{eqnarray*}
    where $p_{ST}$ denotes the probability mass function for $\pbm_{ST}$.
\end{prop}
Note that $H(Law(Y_T),\pbm_{ST})$ is indeed the cross-entropy loss for the classifier $f_{ST}$. Therefore, in actual training, one may use $H(Law(Y_T),\pbm_{ST})\pm\sum_{i=1}^K\log p_{ST}(i)$ to replace   $\Ef^O_\text{KL}(f_{ST})$.

\paragraph{Wasserstein-based output transport risk.}
For learning problems such as GANs or supervised learning with domain adaption, Wasserstein and related distances are popular choices to measure the distance between the generative distribution and the target distribution. Therefore, a Wassertein-based output risk is a natural choice  related to such learning targets. 

More specifically, for $p\geq1$, let $\mathcal{P}_p(\YCal_T)$ be the set of probability measures over $\YCal_T$ such that
\[\int_{\R^{d_{O,T}}}\|x\|_{\YCal_T}^pd\mu(x)<\infty,\quad\forall\mu\in\mathcal{P}_p(\YCal_T).\]
The Wasserstein-based output risk is defined as
\begin{align}\label{eqn:W_risk}
\Ef^O_\text{W}(f_{ST}):=\mathcal{W}_p(\pbm_{ST},\pbm_{T})^p:=\inf_{\gamma\in\Pi(\pbm_{ST},\pbm_{T})}\int_{\R^{d_{O,T}}\times\R^{d_{O,T}}}\|x-y\|_{\YCal_T}^pd\gamma(dx,dy),
\end{align}
for some suitable choice of $p\geq1$, where $\Pi(\pbm_{ST},\pbm_{T})$ denotes the set of couplings of probability measures $\pbm_{ST}$ and $\pbm_{T}$.

 
Analogy to Proposition \ref{lem: kl-heur} is the following property for $\Ef^O_\text{W}(f_{ST})$, based on the triangle inequality of the Wasserstein distance.
\begin{prop}\label{lem: w-heur}
    The Wasserstein-based output risk $\Ef^O_\text{W}$ in (\ref{eqn:W_risk}) is upper bounded in the following sense:
    \[\Ef^O_\text{W}(f_{ST})\leq 2^{p-1}[\mathcal{W}_p(\pbm_{ST},Law(Y_T))^p+\mathcal{W}_p(\pbm_{T},Law(Y_T))^p].\]
\end{prop}
 
Now, consider any intermediate model $f_{ST}$, then Talagrand's inequality 
\cite{talagrand1996transportation} gives 
$$\Ef^I_\text{W}(T_0^X)\leq 2\Ef^I_\text{KL}(T_0^Y),\Ef^O_\text{W}(f_{ST})\leq 2\Ef^O_\text{KL}(f_{ST}).$$
In particular, the linear transfer risk defined in \eqref{eq: risk-ln} satisfies
\begin{align}\label{eqn:risk-ln-KLW}
    \CCal^\lambda_{\text{W}}(S,T|f_{ST})&:=\Ef^O_\text{W}(f_{ST})+\lambda\cdot\Ef^I_\text{W}(T_0^X)\notag\\
    &\leq 2\CCal^\lambda_\text{KL}(S,T|f_{ST}):=2(\Ef^O_\text{KL}(f_{ST})+\lambda\cdot\Ef^I_\text{KL}(T_0^X))
\end{align}
Such a relation between KL- and Wasserstein-based linear transfer risks \eqref{eqn:risk-ln-KLW} gives the following proposition.
\begin{prop}\label{prop: talagrand}
Consider transfer risk in linear form as in \eqref{eqn:risk-ln-KLW}. Suppose $\YCal_T$ is a finite-dimensional Euclidean space and $\pbm_T\ll\pbm_{ST}$. Then for a given transfer learning problem $(S,T,\T_X,\T_Y,\T_X^0,\T_Y^0)$, 
\[\CCal_\text{W}(S,T)\leq 2\CCal_\text{KL}(S,T).\]
\end{prop}



\subsection{Transfer risk and regret}\label{subsec:gaussian}
We will establish the connection between the transfer risk \eqref{eqn:risk} and the transfer learning performance through a linear regression example.

 Consider a source task $S$ and a target task $T$ with the same input space $\XCal_S=\XCal_T=\R^d$ and the same input space $\YCal_S=\YCal_T=\R$. Both source and target data satisfy two $(d+1)$-dimensional Gaussian distributions: $(X_\cdot,Y_\cdot)\sim \mathcal{N}(\mu_\cdot,\Sigma_\cdot)$ with
\begin{equation}\label{eq: source-data}
\mu_\cdot=\begin{pmatrix}\mu_{\cdot,X}\\\mu_{\cdot,Y}\end{pmatrix},\quad \Sigma_\cdot=\begin{pmatrix}\Sigma_{\cdot,X}&\Sigma_{\cdot,XY}\\\Sigma_{\cdot,YX}&\Sigma_{\cdot,Y}\end{pmatrix},
\end{equation}
where
$\mu_{\cdot,Y}\text{ and }\Sigma_{\cdot,Y}\in\R$, $\mu_{\cdot,X}\text{ and }\Sigma_{\cdot,XY}\in\R^d$, $\Sigma_{\cdot,YX}=\Sigma_{\cdot,XY}^\top$, and $\Sigma_{\cdot,X}\in\R^{d\times d}$. Define the sets of admissible source and target models $A_S=A_T=\{f:\R^d\to\R\}$. For any $f\in A_S=A_T$, define the loss function as
\begin{equation}\label{eq: lrloss}
    \LL_S(f)=\E\|Y_S-f(X_S)\|_2^2, \LL_T(f)=\E\|Y_T-f(X_T)\|_2^2.
\end{equation}

Under such a setting, the optimal source and target models are obtained by direct computations: $f_\cdot^*(x)=w_\cdot^\top x+b_\cdot$ with
\begin{align}\label{eq: source-opt}
    w_\cdot=\Sigma_{\cdot,X}^{-1}\Sigma_{\cdot,XY},\quad b_\cdot=\mu_{\cdot,Y}-\Sigma_{\cdot,YX}\Sigma_{\cdot,X}^{-1}\mu_{\cdot,X}.
\end{align}

\paragraph{Transfer learning.} Take the above linear regression example, and consider a simple setting where the input (resp. output) transport set $\mathbb{T}^X$ (resp. $\mathbb{T}^Y$) is a singleton set only containing the identical mapping on $\R^d$ (resp. $\R$). Then, the transfer learning scheme \eqref{eq: doub-trans} is equivalent to directly applying the optimal source model $f^*_S$ to the target task. Consequently, the intermediate model set $\mathcal{I}$ in \eqref{eq: int-set} is also a singleton set with $\mathcal{I}=\{f^*_S\}$. 

Now, define the transfer risk in this linear regression problem as the Wasserstein-based output transport risk as in \eqref{eqn:W_risk}:
\begin{equation}\label{eqn:linear_risk}
\CCal_\text{W}(S,T)=\CCal_\text{W}(S,T|f^*_S)=\Ef^O_\text{W}(f^*_S).
\end{equation}
\paragraph{Regret.} Next, 
define the notion of \textit{regret} as the gap between the transfer learning  and the direct learning:
\begin{equation}\label{eqn:regret}
    \RCal(S,T):=\LL_T(f^*_S)-\LL_T(f^*_T)
\end{equation}
Then, the following proposition shows that the transfer risk serves as a lower bound of the regret.

% $\RCal(S,T):=\LL_T(f_{ST})-\LL_T(f_T)$. Notice that the squared $L_2$ loss in linear regression belongs to a family of Bregman divergence $D_{\phi}:\YCal_T\times\YCal_T\to\R$ with some strictly and differentiable real-valued function $\phi$ over $\YCal_T$, where
% \[D_{\phi}(y,y')=\phi(y)-\phi(y')-\langle\nabla\phi(y'),y-y'\rangle.\]
% \begin{prop}
% \label{coro: regret}
% Suppose the training loss in the target task is a Bregman divergence $D_\phi$ with $\phi$ strictly convex and differentiable, then the regret with respect to the intermediate model $f_{ST}$ and the optimal target model $f_T$ is given by
%     \[
%     \RCal_\phi(S,T)=\E[D_{\phi}(f_T(X_T),f_{ST}(X_T))].
% \]
% \end{prop}

\begin{prop}\label{prop: lb}
    For transfer learning in linear regression with Gaussian data, the regret with respect to the chosen intermediate model $\RCal(S,T)$ in \eqref{eqn:regret} is lower bounded by the Wasserstein-based transfer risk in \eqref{eqn:linear_risk},
    \[\CCal_\text{W}(S,T)\leq \RCal(S,T).\]
\end{prop}
Proposition \ref{prop: lb} suggests that in evaluating the transfer learning scheme \eqref{eq: doub-trans}, transfer risk provides a proper initial indication of its effectiveness, especially for eliminating unsuitable candidate pretrained models or source tasks if the transfer risk is large. 

\subsection{Transfer risk and regret with Gaussian data}\label{app:gaussian}
In this section, we will revisit the example in Section \ref{subsec:gaussian}. The proof of Proposition \ref{prop: lb} will also be presented in this section. In the following discussion, for any spaces $\XCal$ and $\YCal$, we use the notation $\YCal^{\XCal}$ to denote the set of all the functions from $\XCal$ to $\YCal$.

More specifically, consider a transfer learning problem in linear regression where the source and target data are sampled from two Gaussian distributions respectively. 

\subsubsection{Basic case}
Let us first focus on the case where both data sources are of the same dimension. For the source task $S$, the input and the output spaces are $\XCal_S=\R^d$ and $\YCal_S=\R$, respectively. The source data $(X_S,Y_S)\in\XCal_S\times\YCal_S$ is Gaussian distributed such that $(X_S,Y_S)\sim N(\mu_S,\Sigma_S)$ with
\begin{equation}\label{eq: source-data-distrn}
\mu_S=\begin{pmatrix}\mu_{S,X}\\\mu_{S,Y}\end{pmatrix},\quad \Sigma_S=\begin{pmatrix}\Sigma_{S,X}&\Sigma_{S,XY}\\\Sigma_{S,YX}&\Sigma_{S,Y}\end{pmatrix},
\end{equation}
where
$\mu_{S,Y}\text{ and }\Sigma_{S,Y}\in\R$, $\mu_{S,X}\text{ and }\Sigma_{S,XY}\in\R^d$, $\Sigma_{S,YX}=\Sigma_{S,XY}^\top$, and $\Sigma_{S,X}\in\R^{d\times d}$. Take the set of admissible source models $A_S$ to be the set of functions $f:\R^d\mapsto\R$. For any $f\in A_S$, let the source loss function be 
\begin{equation}\label{eq: lr-loss}
    \LL_S(f)=\E\|Y_S-f(X_S)\|_2^2.
\end{equation}
Then the optimal source model 
\begin{equation}\label{eq: lr-opt-prob}
f_S^*\in\argmin_{f\in A_S}\LL_S(f)
\end{equation}
is given by 
\begin{equation}\label{eq: source-opt-model}
    f_S^*(x)=w_S^\top x+b_s,
\end{equation}
 where
 \begin{equation}\label{eq: pretrn-model}
        w_S=\Sigma_{S,X}^{-1}\Sigma_{S,XY}\in\R^d,\quad b_S=\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\mu_{S,X}\in\R.
    \end{equation}
    
Such$f_S^*$ is then used as the pretrained model for the following target task $T$, where the target input and output spaces are the same as in the source task, $\XCal_T=\XCal_S$ and $\YCal_T=\YCal_S$. The target data $(X_T,Y_T)\in\XCal_T\times\YCal_T$ follows a different Gaussian distribution from that in the source data such that $(X_T,Y_T)\sim N(\mu_T,\Sigma_T)$, with
\begin{equation}\label{eq: target-data-distrn}
    \mu_T=\begin{pmatrix}\mu_{T,X}\\\mu_{T,Y}\end{pmatrix},\quad \Sigma_T=\begin{pmatrix}\Sigma_{T,X}&\Sigma_{T,XY}\\\Sigma_{T,YX}&\Sigma_{T,Y}\end{pmatrix},
\end{equation}
where $\mu_{T,Y}\text{ and }\Sigma_{T,Y}\in\R$, $\mu_{T,X}\text{ and }\Sigma_{T,XY}\in\R^d$, $\Sigma_{T,YX}=\Sigma_{T,XY}^\top$, and $\Sigma_{T,X}\in\R^{d\times d}$. 

The set of admissible target models is the same as the in the source task such that $A_T=A_S$. For any $f\in A_T$, let the target loss function be $\LL_T(f)=\E\|Y_T-f(X_T)\|_2^2$. Then similarly to the source task, the optimal target model $f_T^*$ is given by
\begin{equation}\label{eq: opt-target-model}
    f_T^*(x)=w_T^\top x+b_T,\quad \forall x\in\R^d,
\end{equation}
where
\begin{equation}\label{eq: target-opt-param}
    w_T=\Sigma_{T,X}^{-1}\Sigma_{T,XY},\quad b_T=\mu_{T,Y}-\Sigma_{T,YX}\Sigma_{T,X}^{-1}\mu_{T,X}.
\end{equation}
The corresponding output distribution is then given by
\begin{equation}\label{eq: target-pred}
\pbm_T=\E[Y|X]=N(w_T^\top\mu_{T,X}+b_T,w_T^\top\Sigma_{T,X}w_T)=N(\mu_T,w_T^\top\Sigma_{T,X}w_T).
\end{equation}

To initiate transfer learning from the source task $S$ to the target task $T$, consider the sets of input and output transport mappings $\T^X=\{f|f:\XCal_T\to\XCal_S\}$ and $\T^Y=\{f|f:\XCal_T\times\YCal_S\to\YCal_T\}$, with corresponding sets of initial transport mappings $\T^X_0=\{\text{id}_{\XCal_T}\}$, $\T^Y_0=\{\text{id}_{\YCal_S}\}$. Then the set of intermediate models $\ICal$ is a singleton with $\ICal=\{f_{ST}:f_{ST}=f_S^*\}$.

Given the optimal models in both the source task and the target task, specified by \eqref{eq: source-opt-model}-\eqref{eq: pretrn-model} and \eqref{eq: opt-target-model}-\eqref{eq: target-opt-param}, since the data distribution in the target task is given by \eqref{eq: target-data-distrn}, we have
\begin{equation}\label{eq: tl-init-distrn}
        \pbm_{ST}=f_S^*\# N(\mu_{T,X},\Sigma_{T,X})=N(w_S^\top\mu_{T,X}+b_S, w_S^\top\Sigma_{T,X}w_S).
\end{equation}
Notice that $\pbm_T\ll\pbm_{ST}$, therefore the Lebesgue decomposition leads to 
    $\pbm_T=\tilde\pbm_T$, such that
\begin{equation}
    \label{eq: leb-decomp}
    \frac{d\tilde\pbm_T(y)}{d\pbm_{ST}(y)}=h_{ST}(y)=\sqrt\frac{w_S^\top\Sigma_{T,X}w_S}{w_T^\top\Sigma_{T,X}w_T}\exp\left\{\frac{[y-(w_S^\top\mu_{T,X}+b_S)]^2}{2w_S^\top\Sigma_{T,X}w_S}-\frac{[y-(w_T^\top\mu_{T,X}+b)]^2}{w_T^\top\Sigma_{T,X}w_T}\right\}.
\end{equation}
Direct computation leads to the following result.
\begin{itemize}
\item  The KL-based output transfer risk is given by
    \begin{align*}
        \Ef^O_\text{KL}(f_{ST})=&\frac{1}{2}\left\{\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}-\log{\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}}\right.\\
        &\hspace{35pt}\left.{}-1+\frac{\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}\right\}.
    \end{align*}
\item  The Wasserstein-based output transfer risk is given by
    \[\begin{aligned}
        \Ef^O_{\text{W}}(f_{ST})&=\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2\\
        &+\left(\sqrt{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}-\sqrt{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}\right)^2.
    \end{aligned}\]
\end{itemize}
The computation shows that
\begin{itemize}
\item The risk in transfer learning is due to the discrepancy in the data distributions between source and target tasks, even when the source and target data are of matching dimensions and follow the same family of distributions. 

\item In particular, in both the KL and the Wasserstein cases, the output transfer risk can be decomposed into two parts, one being  the variance terms $\text{error}_{\text{v},\cdot}$ determined by the covariance matrices of the source and target data, and the other being the bias terms $\text{error}_{\text{b},\cdot}$ dependent on the difference between the expectations of $\mu_T$ and $\mu_S$.  

To see this, write
\begin{align}
    \Ef^O_\text{KL}(f_{ST})&=\text{error}_{\text{v,KL}}(S,T)+\text{error}_{\text{b,KL}}(S,T),\label{eq: kl-decomp}\\
    \Ef^O_{\text{W}}(f_{ST})&=\text{error}_{\text{v,W}}(S,T)+\text{error}_{\text{b,W}}(S,T),\label{eq: w-decomp}
\end{align}
where
\[\begin{aligned}
    & \text{error}_{\text{v,KL}}(S,T)=\frac{1}{2}\Bigg(\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}\\
    &\qquad\qquad\qquad\qquad\qquad\qquad-\log{\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}}-1\Bigg),\\
    & \text{error}_{\text{b,KL}}(S,T)=\frac{\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2}{2\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}};\\
    & \text{error}_{\text{v,W}}(S,T)=\left(\sqrt{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}-\sqrt{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}\right)^2,\\
    & \text{error}_{\text{b,W}}(S,T)=\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2.
\end{aligned}\]

\item The KL-based variance term 
\[\text{error}_{\text{v,KL}}=h\left(\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}\right),\]
with the function $h:(0,\infty)\to\R$ such that $h(x)=\frac{1}{2}(x-\log x-1)$ for any $x>0$, which is strictly convex and reaches its minimum value $0$ at $x=1$. Thus, for both the KL- and the Wasserstein-based output transfer risks, their variance risk components vanish if and only if
    \[\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}=\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{T,X}\Sigma_{S,X}^{-1}\Sigma_{S,XY}.\]
    
\item The bias risk components $\text{error}_{\text{b,KL}}(S,T)$ and $\text{error}_{\text{b,W}}(S,T)$ remain strictly positive unless the weighted difference between the expectations $\mu_T$ and $\mu_S$ is $0$.
%\end{rmk}
\end{itemize}

\paragraph{Regret analysis.}
By direct computation, one can show that the regret \eqref{eqn:regret} for this linear transfer leaning problem is given by
\begin{equation}\label{eqn:regret_explicit}
    \RCal(S,T)=\|\Sigma^{\frac{1}{2}}(w_T-w_S)\|_2^2+\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2.
\end{equation}
We denote the first term in \eqref{eqn:regret_explicit} as $\hat{\text{error}}_{\text{v}}(S,T):=\|\Sigma^{\frac{1}{2}}(w_T-w_S)\|_2^2$, and denote the second term in \eqref{eqn:regret_explicit} as $\hat{\text{error}}_{\text{b}}(S,T):=\left[\mu_{T,Y}-\mu_{S,Y}-\Sigma_{S,YX}\Sigma_{S,X}^{-1}\left(\mu_{T,X}-\mu_{S,X}\right)\right]^2$.

Recall from \eqref{eqn:linear_risk} that the Wasserstein-based transfer risk for this problem is defined as $\CCal_{\text{W}}(S,T)=\Ef^O_{\text{W}}(f_{ST})$ in \eqref{eq: w-decomp}. Meanwhile, it can be easily verified by comparing \eqref{eq: w-decomp} and \eqref{eqn:regret_explicit} that 
\begin{equation}\label{eqn:compare_risk_regret}
    \RCal(S,T)=\CCal_{\text{W}}(S,T)+2\left(\|\Sigma_{T,X}^{1/2}w_T\|_2\|\Sigma_{T,X}^{1/2}w_S\|_2-\langle\Sigma_{T,X}^{1/2}w_T,\Sigma_{T,X}^{1/2}w_S\rangle\right).
\end{equation}
Proposition \ref{prop: lb} is an immediate consequence of \eqref{eqn:compare_risk_regret} and the Cauchy–Schwarz inequality.

\begin{rmk}
    Proposition \ref{prop: lb} suggests that for evaluating a transfer learning scheme as in \eqref{eq: tl-fw}, transfer risk provides a proper initial indication of its effectiveness, especially when eliminating unsuitable candidate pretrained models or source tasks if the transfer risk is large. Further examining the decomposition of the transfer $\CCal_\text{KL}$ and $\CCal_{\text{W}}$ as well as the regret $\RCal$, we notice that
    \begin{itemize}
        \item A vanishing bias term in transfer risks is equivalent to a vanishing bias term in regret, i.e., $\hat{\text{error}}_{\text{b}}(S,T)=0\Longleftrightarrow \text{error}_{\text{b,KL}}(S,T)=\text{error}_{\text{b,W}}(S,T)=0$
        \item A vanishing variance term in transfer risk is necessary for a vanishing variance term in regret, i.e., $\hat{\text{error}}_{\text{v}}(S,T)=0\Longrightarrow \text{error}_{\text{v,KL}}(S,T)=\text{error}_{\text{v,W}}(S,T)=0$. 
        \item The residual term 
        $$2\left(\|\Sigma_{T,X}^{\frac{1}{2}}w_T\|_2\|\Sigma_{T,X}^{\frac{1}{2}}w_S\|_2-\langle\Sigma_{T,X}^{\frac{1}{2}}w_T,\Sigma_{T,X}^{\frac{1}{2}}w_S\rangle\right)$$
        in \eqref{eqn:compare_risk_regret} depends entirely on the source and target covariance matrices $\Sigma_S$ and $\Sigma_T$is due to the variance term in the learning objective difference. Therefore, when $\CCal_{\text{W}}(S,T)=0$ (or $\CCal_\text{KL}(S,T)=0$), the training process is to reduce the angular distance between $\Sigma_{T,X}^{1/2}w_S$ and $\Sigma_{T,X}^{1/2}w_T$ caused by the discrepancy in these two covariance matrices.
    \end{itemize}
\end{rmk}


\subsubsection{Case with feature augmentation} Let us now consider the  case with feature augmentation. That is, compared with the input data in the source task, the target task includes more input information in the form of a higher input dimension. 
We will see that potential extra transfer risk as a result of the extra augmented  input information as well as its benefit to eliminate the bias risk.

Take the same source task $S$ as in the basic case; for the target task $T$, let the input space  $\XCal_T=\R^{d+k}$ with $k\in\mathbb{N}^+$, let  the output space be the same as in the target task $T$ such that $\YCal_T=\YCal_S=\R$. Since the transfer learning problem has a feature augmentation, let us first define a projection  $\XCal_T$ from $T^X_0$ to $\XCal_S$ such that 
\[T^X_0(x)=\begin{pmatrix}I_d&\vdots&O_{d\times k}\end{pmatrix}x,\quad\forall x\in\XCal_T.\]
Then the target data $(X_T,Y_T)\in\XCal_T\times\YCal_T$ satisfies that
$T^X_0(X_T)=X_S$ and $Y_T=Y_S$. That is, $(X_T,Y_T)$ is given by a Gaussian distribution $N(\mu_T,\Sigma_T)$ with $\mu_T$ and $\Sigma_T$ in the same form as in \eqref{eq: target-data-distrn}, where
\begin{align*}
&\mu_{T,X}=\begin{pmatrix}\mu_{S,X}\\\mu_{A,X}\end{pmatrix},\quad  \mu_{T,Y}=\mu_{S,Y},\\ 
&\Sigma_{T,X}=\begin{pmatrix}\Sigma_{S,X} & \Sigma_{AS,X}\\ \Sigma_{AS,X}^\top & \Sigma_{A,X}\end{pmatrix},\quad \Sigma_{T,XY}=\begin{pmatrix}\Sigma_{S,XY}\\\Sigma_{A,XY}\end{pmatrix},\quad \Sigma_{T,Y}=\Sigma_{S,Y}.
\end{align*}
Here $\mu_{A,X}\in\R^k$ denotes the expectation of the augmented variable $\tilde X_T$ such that $X_T^\top=\begin{pmatrix}
    T^X_0(X_T)^\top&\tilde X_T^\top
\end{pmatrix}$; in the above covariance matrix $\Sigma_T$, $\Sigma_{AS,X}=\text{Cov}(X_S,\tilde X_T)\in\R^{d\times k}$, $\Sigma_{A,X}=\text{Var}(\tilde X_T)\in\R^{k\times k}$, and $\Sigma_{A,XY}=\text{Cov}(\tilde X_T,Y_T)\in\R^{k}$.
The optimal linear model $f_T^*$ is again given by \eqref{eq: opt-target-model}-\eqref{eq: target-opt-param} with the optimal parameters $w_T$ and $b_T$ re-computed under the above modified target data distribution. The corresponding output distribution $\pbm_T$ is of the form \eqref{eq: target-pred} with updated parameters as in $f_T^*$.

To initialize the transfer learning problem from $S$ to $T$, consider $\T^X_0=\{T^X_0\}$, $\T^Y_0=\{\text{id}_{\YCal_S}\}$, $\T^X=\{f|f:{\XCal_T}\to\XCal_S\}$, and $\T^Y=\{f|f:\XCal_T\times\YCal_S\to\YCal_T\}$. The set of intermediate models $\ICal$ is still singleton, with $\ICal=\{f_{ST}:f_{ST}=f_S^*\circ T^X_0\}$. Clearly,  $\pbm_{ST}=Law(f_S^*(X_S))$, with $\pbm_T\ll Law(f_S^(X_S))$.
Now we have
  \begin{itemize}
  \item The KL-based output transfer risks are given by 
    \begin{equation}\label{eq: kl-or-ia}
        \Ef^O_\text{KL}(f_{ST})=\frac{1}{2}\left[\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}-\log{\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}}-1\right];
\end{equation}
\item The  Wasserstein-based output transfer risk is 
\begin{equation}
        \Ef^O_{\text{W}}(f_{ST})=\left(\sqrt{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}-\sqrt{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}\right)^2.
    \end{equation}
\end{itemize}

Comparing the basic case and  this feature augmentation case, we see
\begin{itemize}
\item The extra input information enables the particular choice of the initial input and output transport mappings, $T^X_0$ and $\text{id}_{\YCal_S}$, which in turn  eliminates the bias risk component in both the KL- and Wasserstein-based output risk. 
\item Both output transfer risks come from their corresponding variance risk component. Take the KL-based output transfer risk in \eqref{eq: kl-or-ia} as an example. We see that 
\[\Ef^O_\text{KL}(f_{ST})=\text{error}_{\text{v,KL}}(S,T)=h\left(\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}\right).\]
This suggests that the challenge of applying transfer learning with feature augmentation lies mainly at the uncertainty from the augmented variable $\tilde X_T$. 
\item In particular, if one assumes that the added input information $\tilde X_T$ is uncorrelated with the existing input data $X_S$, then 
\[\frac{\Sigma_{T,YX}\Sigma_{T,X}^{-1}\Sigma_{T,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}=1+\frac{\Sigma_{A,YX}\Sigma_{A,X}^{-1}\Sigma_{A,XY}}{\Sigma_{S,YX}\Sigma_{S,X}^{-1}\Sigma_{S,XY}}.\]
That is, when one introduces new features that are uncorrelated with the existing ones, the variance risk component is always positive unless these new features are also uncorrelated with the output.

\end{itemize}

\subsubsection{Case with augmented output space}
Let us now consider the case with an extra prediction task, i.e.,  a transfer learning problem with augmented output space. 
In this case, we will  see extra transfer risk with two major contributing factors, one being the unforeseeable correlation between the input and the extra output information and the other being the necessary initialization procedure due to the extra task in the target task. 

To see this, let us consider a source task  slightly modified from the basic case, where the output space in $S$ is allowed be of dimension bigger that $1$, that is, $\YCal_S=\R^l$ with $l\in\mathbb{N}^+$. Then the source data $(X_S,Y_S)$  is given by a Gaussian distribution $N(\mu_S,\Sigma_S)$ with $\mu_S$ and $\Sigma_S$ as in \eqref{eq: source-data-distrn} except that $\mu_{S,Y}\in\R^l$, $\Sigma_{S,XY}\in\R^{d\times l}$ and $\Sigma_{S,Y}\in\R^{l\times l}$. Again the optimal linear model $f_S^*$  is given by \eqref{eq: source-opt-model}-\eqref{eq: pretrn-model} with optimal parameters $w_S$ and $b_S$ re-computed under the above modified source data distribution. 

For the target task, let $\XCal_T=\XCal_S$ and $\YCal_T=\R^{l+k}$ with $k\in\mathbb{N}^+$. Since the transfer learning problem has an extra learning task with the same input data, the target data $(X_T,Y_T)\in\XCal_T\times\YCal_T$ satisfies that $X_T=X_S$ and $Y_T^\top=\begin{pmatrix}Y_S&Y_A\end{pmatrix}^\top$ from some random variable $Y_A\in\R^K$. Let us assume that the joint distribution of the input and output variables $(X_T,Y_T)$ follows a Gaussian distribution $N(\mu_T,\Sigma_T)$ with $\mu_T$ and $\Sigma_T$ in the same form as in \eqref{eq: target-data-distrn}, where
\[\begin{aligned}
    &\mu_{T,Y}=\begin{pmatrix}\mu_{S,Y}\\\mu_{A,Y}\end{pmatrix},\quad \mu_{T,X}=\mu_{S,X},\\
    &\Sigma_{T,Y}=\begin{pmatrix}\Sigma_{S,Y} & \Sigma_{AS,Y}\\\Sigma_{AS,Y}^\top & \Sigma_{A,Y}\end{pmatrix},\quad \Sigma_{T,YX}=\begin{pmatrix}\Sigma_{S,YX}\\ \Sigma_{A,YX}\end{pmatrix},\\ &\Sigma_{T,XY}=\begin{pmatrix}\Sigma_{S,XY} & \Sigma_{A,XY}\end{pmatrix},\quad \Sigma_{T,X}=\Sigma_{S,X}.
\end{aligned}\]
Here $\mu_{A,Y}=\E[Y_{A}] \in\R^k$ denotes the expectation of $Y_A$, $\Sigma_{AS,Y}=\text{Cov}(Y_S,Y_A)\in\R^{l\times k}$, $\Sigma_{A,Y}=\text{Var}(Y_A)\in\R^{k\times k}$ and $\Sigma_{A,XY}=\Sigma_{A,YX}^\top=\text{Cov}(X_S,Y_A)\in\R^{d\times k}$. 
Then again the optimal linear model $f_T^*$ is in the form of \eqref{eq: opt-target-model}
with parameters
\[\begin{aligned}
    w_T^\top&=\Sigma_{T,YX}\Sigma_{T,X}^{-1}=\begin{pmatrix}\Sigma_{S,YX}\Sigma_{S,X}^{-1}\\\Sigma_{A,YX}\Sigma_{S,X}^{-1}\end{pmatrix}=\begin{pmatrix}w_S^\top\\\Sigma_{A,YX}\Sigma_{S,X}^{-1}\end{pmatrix},\\ 
    b_T&=\mu_{T,Y}-\Sigma_{T,YX}\Sigma_{T,X}^{-1}\mu_{T,X}=\begin{pmatrix}\mu_{S,Y}\\\mu_{A,Y}\end{pmatrix}-\begin{pmatrix}\Sigma_{S,YX}\Sigma_{S,X}^{-1}\mu_{S,X}\\\Sigma_{A,YX}\Sigma_{S,X}^{-1}\mu_{S,X}\end{pmatrix}\\
    &=\begin{pmatrix}b_S\\\mu_{A,Y}-\Sigma_{A,YX}\Sigma_{S,X}^{-1}\mu_{S,X}\end{pmatrix}.\end{aligned}\]
Correspondingly, $\pbm_T=\E[Y_T|X_T]=N\left(\mu_1,\Sigma_1\right)$, where
\[\begin{aligned}
\mu_1&=w_T^\top\mu_{T,X}+b_T=\begin{pmatrix}w_S^\top\mu_{S,X}+b_S\\\mu_{A,Y}\end{pmatrix},\\
\Sigma_1&=w_T^\top\Sigma_{T,X}w_T=\begin{pmatrix}w_S^\top\Sigma_{S,X}w_S & w_S^\top\Sigma_{A,XY}\\\Sigma_{A,YX}w_S & \Sigma_{A,YX}\Sigma_{S,X}^{-1}\Sigma_{A,XY}\end{pmatrix}.
\end{aligned}\]

To initialize the transfer learning, consider the sets of input and output transport mappings $\T^X=\{f|f:\XCal_T\to\XCal_S\}$ and $\T^Y=\{f|f:\XCal_T\times\YCal_S\to\YCal_T\}$, as well as the sets of initial input transport mappings $\T^X_0=\{\text{id}_{\XCal_T}\}$. For the initial output mapping, in order to handle the newly added prediction task from $X_T=X_S$ to $Y_A$, let us define an initial function $f_0:\R^d\to\R^k$ as $f_0(x)=w_0^\top x+b_0$ for any $x\in\R^d$ with fixed $w_0\in\R^{k\times d}$ and $b_0\in\R^k$. The set of initial output transport mappings is given by 
$$\T^Y_0=\left\{T^Y_0:\XCal_T\times\YCal_S\to\YCal_T|T^Y_0(x,y)=\begin{pmatrix}y^\top&\vdots&f_0(x)^\top\end{pmatrix}^\top\right\}.$$
Once again, the set of intermediate models $\ICal$ is a singleton with 
$$\ICal=\{f_{ST}: f_{ST}(x)=T^Y_0(x,f_S^*(x)),\,\forall x\in\XCal_T\}.$$
The probability distribution $\pbm_{ST}$ of the intermediate model $f_{ST}$ is given by $\pbm_{ST}=N(\mu_2,\Sigma_2)$, where
\[\begin{aligned}    &\mu_2=\begin{pmatrix}w_S^\top\\w_0^\top\end{pmatrix}\mu_{T,X}+\begin{pmatrix}b_S\\b_0\end{pmatrix}=\begin{pmatrix}w_S^\top\mu_{S,X}+b_S\\w_0^\top\mu_{S,X}+b_0\end{pmatrix},\\
    &\Sigma_2=\begin{pmatrix}w_S^\top\\w_0^\top\end{pmatrix}\Sigma_{T,X}\begin{pmatrix}w_S & w_0\end{pmatrix}=\begin{pmatrix}w_S^\top\Sigma_{S,X}w_S& w_S^\top\Sigma_{S,X}w_0\\w_0^\top\Sigma_{S,X}w_S & w_0^\top\Sigma_{S,X}w_0\end{pmatrix}.
\end{aligned}\]
We have again $\pbm_T\ll\pbm_{ST}$, and 
\begin{itemize}
 \item    The KL- 
 and Wasserstein-based output transfer risks are given by 
    \begin{equation}
        \Ef^O_\text{KL}(f_{ST})=\frac{1}{2}\left[Tr(\Sigma_2^{-1}\Sigma_1)-\log{\frac{\text{det}(\Sigma_1)}{\text{det}(\Sigma_2)}}-(k+l)+(\mu_1-\mu_2)^\top\Sigma_2^{-1}(\mu_1-\mu_2)\right];\label{eq: kl-or-oa}
        \end{equation}
      \item The Wasserstein-based output transfer risk is  given by
      \begin{equation}
        \Ef^O_{\text{W}}(f_{ST})=\|\mu_1-\mu_2\|_2^2+Tr\left(\Sigma_1+\Sigma_2-2\left(\Sigma_1^{\frac{1}{2}}\Sigma_2\Sigma_1^{\frac{1}{2}}\right)^{\frac{1}{2}}\right).
    \end{equation}
\end{itemize}
The analysis shows that with the augmented output space, the output transfer risks vanish if the initialization function $f_0$ can neutralize the uncertainty brought by the correlation between the input $X_S$ and the additional output information $Y_A$. 

To see this, take the example of the KL-based output transfer risk in \eqref{eq: kl-or-oa}, and decompose $\Ef^O_\text{KL}(f_{ST})$ in \eqref{eq: kl-or-oa} into its variance and bias components as in \eqref{eq: kl-decomp}, with
\[\begin{aligned}
    & \text{error}_{\text{v,KL}}(S,T)=\frac{1}{2}Tr(\Sigma_2^{-1}\Sigma_1)-\log{\frac{\text{det}(\Sigma_1)}{\text{det}(\Sigma_2)}}-(k+l),\\
    & \text{error}_{\text{b,KL}}(S,T)=\frac{1}{2}(\mu_1-\mu_2)^\top\Sigma_2^{-1}(\mu_1-\mu_2).
\end{aligned}\]
Now, we see that
\begin{itemize}
    \item If $0<\lambda_1\leq\dots\leq\lambda_{k+l}$ are the eigenvalues of $\Sigma_2^{-1}\Sigma_1$, and if $\Sigma_1$ and $\Sigma_2$ are invertible. Then the variance term can be written as
    \[
        \text{error}_{\text{v}}(S,T)=\sum_{i=1}^{k+l}(\lambda_i-\log\lambda_i-1)\geq0, 
    \]
    which vanishes if and only if $\lambda_i$'s are all equal to $1$ such that $\Sigma_1=\Sigma_2$.

    \item The difference between the expectations of $\pbm_T$ and $\pbm_{ST}$  is given by
    \[\mu_1-\mu_2=\begin{pmatrix}0\\\mu_{A,Y}-w_0^\top\mu_{S,X}-b_0\end{pmatrix}.\]
    Therefore, the error between the expected augmented output $\mu_{A,Y}$ and $w_0^\top\mu_{S,X}+b_0$ derived from the chosen initialization $f_0$ is the main contributor to a strictly positive bias risk component $\text{error}_{\text{b,KL}}$. 
\end{itemize}
